Repeton: Structured Bug Repair with ReAct-Guided Patch-and-Test Cycles

Large Language Models (LLMs) have shown strong capabilities in code generation and comprehension, yet their application to complex software engineering tasks often suffers from low precision and limited interpretability. We present Repeton, a fully open-source framework that leverages LLMs for precise and automated code manipulation in real-world Git repositories. Rather than generating holistic fixes, Repeton operates through a structured patch-and-test pipeline: it iteratively diagnoses issues, proposes code changes, and validates each patch through automated testing. This stepwise process is guided by lightweight heuristics and development tools, avoiding reliance on embedding-based retrieval systems. Evaluated on the SWE-bench Lite benchmark, our method shows good performance compared to RAG-based methods in both patch validity and interpretability. By decomposing software engineering tasks into modular, verifiable stages, Repeton provides a practical path toward scalable and transparent autonomous debugging.

==> contents/3_method_old.tex <==
\section{Method}

We propose a modular stepwise debugging pipeline that enables a software agent to autonomously identify, localize, and resolve bugs in software projects. Our method is designed to be lightweight, avoiding the use of heavy embedding models, and operates in real time with full interpretability. Figure~\ref{fig:pipeline} illustrates the complete flow of the agent's behavior.

\subsection{Problem Understanding and Reproduction}

Given a software project and a problem description (for example, error logs, user reports, or test failures, etc.), the agent begins by generating a concise summary of the issue. This summary is used to initiate the debugging process. The agent then attempts to reproduce the bug in a controlled environment. If the bug is not reproducible, the process is terminated. Otherwise, the agent proceeds to locate the source of the bug.

\subsection{Keyword Extraction and File Selection}

To begin code-level analysis, the agent extracts a set of relevant keywords from the problem description. These keywords are used to search through the project directory and identify potentially relevant source files. If no relevant files are found, the keyword list is refined and the search is repeated.

\subsection{Code Localization}

Once relevant files are identified, the agent performs a line-by-line search within those files to locate code segments related to the extracted keywords. If no relevant code is found, the agent backtracks and updates its search heuristics. Otherwise, it moves forward to bug fixing.

\subsection{Bug Fixing and Verification}

After isolating the relevant code, the agent generates candidate fixes using domain-specific heuristics or prompt-based reasoning. These fixes are applied to the codebase and the agent attempts to reproduce the bug again to verify the effectiveness of the patch. If the bug persists, the agent iterates through the pipeline with updated hypotheses.

\subsection{Termination Conditions}

The process terminates under one of the following conditions:
\begin{itemize}
    \item The bug is no longer reproducible (considered \textit{Fixed}).
    \item The agent determines that it cannot generate a fix (considered \textit{Cannot fix}).
    \item No relevant code or files can be located after an exhaustive search.
\end{itemize}

This approach allows the agent to maintain a real-time interpretable debugging loop without relying on large embedding models or external indexing systems.
